What Stops Learning-based 3D Registration from Working in the Real World?

Much progress has been made on the task of learning-based 3D point cloud registration, with existing methods yielding outstanding results on standard benchmarks, such as ModelNet40, even in the partial-to-partial matching scenario. Unfortunately, these methods still struggle in the presence of real data. In this work, we identify the sources of these failures, analyze the reasons behind them, and propose solutions to tackle them. We summarise our findings into a set of guidelines and demonstrate their effectiveness by applying them to different baseline methods, DCP and IDAM. In short, our guidelines improve both their training convergence and testing accuracy. Ultimately, this translates to a best-practice 3D registration network (BPNet), constituting the first learning-based method able to handle previously-unseen objects in real-world data. Despite being trained only on synthetic data, our model generalizes to real data without any fine-tuning, reaching an accuracy of up to 67% on point clouds of unseen objects obtained with a commercial sensor.

==> fig/tudl_qual.tex <==
\begin{figure}[!ht]
    \centering
    \includegraphics[width=3.8cm]{image/robot.png}
    \caption{\label{tudl_qual} Qualitative results on the TUDL dataset. \ZD{(placeholder)}}
\end{figure}

==> fig/visible_surface.tex <==
\begin{figure}[!ht]
    \centering
    \includegraphics[width=3.8cm]{image/visible_surface_sampling.pdf}
    \caption{\label{visible_surface} Visible Surface Sampling \ZD{(placeholder)}}
\end{figure}

==> table/baseline_result.tex <==
\begin{table}[!htb]
    \centering
    {\footnotesize
    \setlength{\tabcolsep}{2.5mm}{
    \begin{tabular}{l|ccc|ccc}
        \toprule
        & \multicolumn{3}{c|}{Rotation mAP} & \multicolumn{3}{c}{Translation mAP} \\
        Method & $5^{\circ}$ & $10^{\circ}$ & $15^{\circ}$ & $2cm$ & $5cm$ & $10cm$\\
        \midrule
        Baseline-A    & 90.45 & 90.45 & 90.45 & 3.28 & 2.50 & 2.27 \\
        Baseline-B    & 90.45 & 90.45 & 90.45 & 3.28 & 2.50 & 2.27 \\
        Baseline-C    & 90.45 & 90.45 & 90.45 & 3.28 & 2.50 & 2.27 \\
        \bottomrule
    \end{tabular}
    }}
    \caption{Baseline result: place holder, A:full object pose estimation, B: partial-to-partial pointcloud matching, C:self-occluded object pose estimation(real scene)}
    \label{tab:baseline_result}
\end{table}

==> table/visible_surface_sampling.tex <==
\begin{table*}[!htb]
    \centering
    {\footnotesize
    \setlength{\tabcolsep}{4.5mm}{
    \begin{tabular}{l|cccc|cccc}
        \toprule
        & \multicolumn{4}{c|}{Rotation mAP} & \multicolumn{4}{c}{Translation mAP} \\
        Method & $5^{\circ}$ & $10^{\circ}$ & $15^{\circ}$ & $20^{\circ}$ & 0.001 & 0.005 & 0.01 & 0.05 \\
        \midrule
        OPRNet+RTD    & 90.45 & 90.45 & 90.45 & 3.28 & 2.50 & 2.27 & 9.50 & 7.99  \\
        \rowcolor{mapillarygreen}
        OPRNet+VRA & 89.61 & 83.80 & 70.84 & 8.26 & 6.15 & 6.06 & 13.10 & 11.12  \\
        \bottomrule
    \end{tabular}
    }}
    \caption{Effectiveness of Visible Surface Sampling.}
    \label{tab:tudl_2}
\end{table*}

==> tex/baseline.tex <==
\input{table/baseline_result}

\section{Baseline Model}

We choose DCP(v2) to be our baseline model not just for its simplicity, but also for it provides a pipeline includes modern techniques and will be used for comparison. In the following section, we're going to reveal the full potential of the DCP method by changing a small amount but necessary component.

Since the original DCP method was designed to estimate the relative transformation between two fully observed pointcloud, it means the original DCP neither can handle the partial-to-partial pointcloud matching nor the self-occluded object pose estimation task. However, in the following section, we're going to show with the changes of three most crucial components, the DCP will first gain the power to handle wide rotation range, then able to handle the partial-to-partial pointcloud registration well and finally able to handle the self-occluded object pose estimation task even evaluated on the real scene data without any fine-tuning.

% \subsection{Baseline Method}

% We use DCP(v2) as our baseline method, but with few changes:

% \paragraph{1. input reduce mean.}
% Since the target pointcloud could be far from the camera then has a large magnitude of the value in the xyz. Here we reduce the mean on each axis to move the target pointcloud in a $[-1,1]$ cube. This move could be consider as normalization on the translation axis. After the estimation of the translation we add back the reduced mean. Since this is a small but crutial point we make it as the default setting. 

% \paragraph{2. remove the moving mean and var in the batch normalization.}
% In practice we found this achieve better performance, thus we keep this part as the default setting.

% \paragraph{3. optimizer change to be adam without scheduler.}
% The original DCP using a scheduler to control the learning rate, however, we found this part affect little on the performance. In order to keep the simplicity, we using the Adam with a fixed learning rate.

\subsection{Baseline Result}

Here we list three experiments each corresponding to different task. To be specific, the first one is the full object pointcloud registration task, the second one is the partial-to-partial pointcloud registration task, the last one is the real scene self-occluded object pose estimation task.

The result are summarize in the table~\ref{tab:baseline_result}


% ------------------------------------------------------------------------



% \input{fig/visible_surface}
% \input{fig/pipeline_compare}

% \subsection{Preliminary knowledge}

% Before we introduce our proposed method, here we review the widely used non-viewpoint rendering augmentation first. As done by e.g. PointnetLK DCP, which were designed to work under the unrealistic assumption that both point sets are fully observed, even at the test time, follow-up works focused on the more practical partial-to-partial registration scenario PRNet, RPMNet. Nevertheless, these techniques still assume the observations to depict a point-cloud in full 3D. To be specific, they take the fully observed 3D mesh model, sampling from the mesh model and then using two plane to slice the pointcloud into two pieces which have overlapped area. They called this kind of task to be partial-to-partial pointcloud matching. At first glance, the real scene case seems like just the sub task of this partial-to-partial pointcloud matching. But there are several things need to be noticed.

% 1. The object in the partial-to-partial pointcloud matching can be see through the inner structure, but in the self-occluded case is not. Some mesh model contains the inner structure, for example, a car with seats inside. If the seat can be observed, the partial-to-partial matching will have more matching point in the overlapping area, but these seats' pointcloud cannot be observed by the depth sensor, thus cannot find the corresponding point in the target pointcloud. Thus making the self-occluded task harder.

% 2. The noise in the partial-to-partial pointcloud matching is only Gaussian noise, but in the self-occluded case is not. In the self-occluded case, the mis-alignment of two point can be cause by the discrete sampling of the depth map. This kind of noise is cause by the imaging principle of camera, even create by the rendering also can not be avoid. Thus the error is system error, there is no guarantee that model trained with Gaussian noise can work on self-occluded task.

% 3. The partial-to-partial pointcloud matching's overlapping can be controled, but the self-occluded cannot. In the real scene scenario, if a guitar be observed from the front the overlapping area with the mesh model is close to 50\%. However, if it's been observed from the right-side, it looks like a slender rectangle. In this case the overlapping area is below 10\%. Thus make the self-occluded task harder.

% % 4. The partial-to-partial task slices the object's pointcloud making \textbf{all} the training and testing object asymmetrical, which reduced the difficulty. However, slicing the mesh model will left the smooth plane, which could induce the ambiguity when observing one object from a certain view, as a result making the self-occluded task to be more challenging.
% 4. The partial-to-partial task test with limited rotation range, to be specific, $[0, 45^{\circ}]$. However, in the real scene dataset the rotation range is wider than this, which is full rotation range. 

% 5. The last but not the least, the model which train with partial-to-partial augmentation cannot be directly used to solve self-occluded task.

% Comparing with the traditional RGB or RGB-D based 6D pose estimation task:

% 1. Traditional 6D pose estimation task focus on the known objects, but our task focus on generalization to unseen objects. In the traditional 6D pose task, the training and testing objects are the same, but in our task, the testing models are different from training models. This setting is non-trivial. 
% Since the XXX, XXX assume that the network could acquire enough knowledge about how to estimate the target object in the fixed coordinate reference system, thus in the training and testing process only takes the RGB or RGB-D images and predicts the 3D coordinates of the corner of the bounding box of object in the object coordinate system, like in the paper BB8. Then using PnP to get the final estimation of the pose. As for the RGB-D method, they using ICP for the final refinement. 
% In this case, if two objects' appearance are similar, but been placed in different direction in the reference system, the network could be confused. However, in our task, since we take both source and target pointcloud, thus this problem could be resolved. This setting makes our task is suitable for the unseen object pose estimation, whereas the traditional task setting are not.

% 2. The traditional 6D pose estimation task use the real scene data for fine-tuning, as in the paper CosyPose, but our task only use the object's mesh model. In the traditional setting, they use synthetic data for pre-training and fine-tune the model on both real and synthetic images or just real images. In our setting, we only take the synthetic mesh model as input, and evaluate our algorithm on the real scene data. Not mention our task also have to generalize to the unseen objects, the arduousness of our task is self-evident.

% 3. Our method is the first depth-based learning method on the unseen object 6D pose estimation task.

% 4. The real scene data is limited, thus pose a negative effect in the training process. However, with the propose viewpoint rendering augmentation, we can have infinity training sample, this problem can be fixed. \zd{From the experiment we show that the model trained with our viewpoint rendering augmentation is even better than using the real scene data.}

% \subsection{Viewpoint Rendering Augmentation}

% 1. Normalize the model.

% To introduce the core work of this paper, the viewpoint rendering augmentation, we need to get an idea about the estimating the 6D pose of the object of interest first. To this end, let $\bX \in \mathbb{R}^{M \times 3}$ and $\bY \in \mathbb{R}^{N \times 3}$ be two sets of 3D points sampled from the same object surface. We typically refer to $\bX$ as the source point set and to $\bY$ as the target point set. 
% % We obtain the source point set $\bX$ by visible surface sampling strategy~\ref{visible_surface} instead of uniform sampling from the mesh model which used in the paper DCP, RPMNet\ZD{add more paper}.
% We obtain the source point set $\bX$ through uniform sampling from the mesh model.
% The target one $\bY$ is obtained from $I_{depth}$ and $I_{mask}$, assuming known camera intrinsic parameters. Registration then aims to find a rigid transformation $\bT$ that aligns $\bX$ to $\bY$. In this work, we focus on the case where the object is self-occluded. To be specific, we assume that each point in $\bY$ has a corresponding point in $\bX$, but not the opposite.

% \paragraph{Combine with OPRNet Backbone.}

% The OPRNet backbone consists of a DGCNN~\cite{Wang18b} followed by a Transformer~\cite{Vaswani17}. Specifically, the DGCNN takes a point set as input, constructs a k-NN graph from it, and then extracts point-wise features via standard convolutions on this graph, encoding diverse levels of context by max-pooling the local features and concatenating the resulting representations to the point-wise ones.
% Let $\bthx$, resp. $\bthy$, be the final feature matrix, i.e., one $P$-dimensional feature vector per 3D point, for $\bX$, resp. $\bY$. The transformer then learns a function $\phi : \mathbb{R}^{M\times P} \times \mathbb{R}^{N\times P} \rightarrow \mathbb{R}^{M\times P}$, that combines the information of the two point sets. Ultimately, this produces descriptor matrices $\bfx$, resp. $\bfy$, for $\bX$, resp. $\bY$, written as
% \begin{equation}
%     \bfx = \bthx + \phi(\bthx, \bthy), \;\;\;
%     \bfy = \bthy + \phi(\bthy, \bthx)\;.
% \end{equation}
% Given these matrices, the OPRNet forms a score map $\bS \in \mathbb{R}^{M\times N}$ by computing the similarity between each source-target pair of descriptors. That is, we compute the $(i,j)$-th element of $\bS$ as
% \begin{equation}
%     \bS_{i,j} = <\bfx_i, \bfy_j>, \;\;\forall (i, j) \in [1,M]\times [1,N]\;,
% \end{equation}
% where $<\cdot, \cdot>$ is the inner product, and $\bfx_i, \bfy_j \in \mathbb{R}^P$. To handle the outlier and noise caused mismatch, the OPRNet adopts the Optimal Transport Layer~\cite{}. Specifically, it extends the score matrix $\bS$ by one row and one column to form an augmented score matrix $\bbS$. The values at the newly-created positions in $\bbS$ are set to
% \begin{equation}
%     \bbS_{i, N + 1} = \bbS_{M + 1, j} = \bbS_{M + 1, N + 1} = \alpha,
% \end{equation}
% $\forall i \in [1, M], \;\forall j \in [1, N]$, where $\alpha \in \mathbb{R}$ is a fixed parameter, which set to be $0.01$ in practice. The values at the other indices directly come from $\bS$. Given the augmented score map $\bbS$, we aim to find a partial assignment $\bbP \in \mathbb{R}^{(M+1)\times (N+1)}$, defining correspondences between the two point sets, extended with the outlier bins.

% In OPRNet, the supervision is directly imposed on the output of the Optimal Transportation Layer.
% To this end, let $\bM \in \{0, 1\}^{M \times N}$ be the matrix of ground-truth correspondences, with a $1$ indicating a correspondence between a pair of points. Such correspondences can be estimated using the ground-truth transformation matrix. To build the ground-truth assignment matrix $\bM$, as introduced in the OPRNet paper, we transform $\bX$ using the ground-truth transformation $\bT$, giving us $\btX$. We then compute the pairwise Euclidean distance matrix between $\btX$ and $\bY$, which we threshold to $0.05$ to obtain a correspondence matrix $\bM \in \{0, 1\}$. OPRNet augments $\bM$ with an extra row and column acting as outlier bins to obtain $\bbM$. The points without any correspondence are treated as outliers, and the corresponding positions in $\bbM$ are set to one. This strategy does not guarantee a bipartite matching, which OPRNet addresses using a forward-backward check. We keep using the loss function which used in the OPRNet, to be specific, the loss function is expressed as the negative log-likelihood

% \begin{equation}
%     \mathcal{L}(\bP, \bbM) = \frac{- \sum\limits_{i =1}^{M+1}\sum\limits_{j = 1}^{N+1} (\log \bP_{i,j})\bbM_{i, j}}{\sum\limits_{i = 1}^{M+1}\sum\limits_{j = 1}^{N+1} \bbM_{i, j}}\;,
%     \label{eq:nll}
% \end{equation}

% where $\bP$ is the output of the Optimal Transport Layer, and where the denominator normalizes the loss value so that different training samples containing different number of correspondences have the same influence in the overall empirical risk.

% \paragraph{Combine with IDAM Backbone.}

% We implement the viewpoint rendering augmentation using Pytorch3D. We generate scenes that contain individual object without background.

% \paragraph{Comparing to the Pointcloud Slicing Method.}


% \paragraph{Comparing to the real scene data.}


% \subsection{Visible Surface Sampling}
% \label{visible_surface}

% Some of the synthetic mesh models used in the training process have the inner structure, such as the seats in the car as shown in the Fig.\ZD{add the figure}. In this case, if we uniform sampling from the mesh model, the pointcloud of the inner structure will never found the corresponding point in the target point cloud. Thus here we introduce the visible surface sampling strategy, which sampling the points from the mesh model's visible surface. To be specific, we put the camera at the same place and rotating the object to 16 different angle. In this process we render the object's depth map and turn it back to the pointcloud by using camera parameter. We combine these 16 pointclouds to get final surface sampling pointcloud.

% And we found this module is very important when asymmetrical object augmentation is enable. 


% \subsection{Asymmetrical Object Augmentation}

% The symmetrical object been observed from different viewpoint can have same appearance. In the training process, the network takes the same input, but the loss is different. This ambiguity will interrupt the training and testing performance of the network.\ZD{Here we can use a comparison experiment to justify this statement. 500 asymmetrical object and 500 symmetrical object for training and evaluate on the asymmetrical clear dataset.}

% To eliminate the ambiguity in the training process bring by the symmetrical object, we introduce the asymmetrical object augmentation. To be specific, we add a sphere and a octahedron to merge with the object mesh model which its center be placed at the surface of the object. As shown in the figure, the octahedron and the sphere have been placed at the different place of the cup, thus make the symmetrical object asymmetrical. To be noticed, when merging two objects, if still sampling from the mesh model, the overlapping area which is hiding behind the surface also will be sampled. These points also cannot find the corresponding point in the target point cloud, which will make overlapping ratio lower. In this case, the use of 
% asymmetrical augmentation will not only fail to improve performance, but will further reduce performance.
